Cross-View Image Set Geo-Localization

Cross-view geo-localization (CVGL) has been widely applied in fields such as robotic navigation and augmented reality. Existing approaches primarily use single images or fixed-view image sequences as queries, which limits perspective diversity. In contrast, when humans determine their location visually, they typically move around to gather multiple perspectives. This behavior suggests that integrating diverse visual cues can improve geo-localization reliability. Therefore, we propose a novel task: Cross-View Image Set Geo-Localization (Set-CVGL), which gathers multiple images with diverse perspectives as a query set for localization. To support this task, we introduce SetVL-480K, a benchmark comprising 480,000 ground images captured worldwide and their corresponding satellite images, with each satellite image corresponds to an average of 40 ground images from varied perspectives and locations. Furthermore, we propose FlexGeo, a flexible method designed for Set-CVGL that can also adapt to single-image and image-sequence inputs. FlexGeo includes two key modules: the Similarity-guided Feature Fuser (SFF), which adaptively fuses image features without prior content dependency, and the Individual-level Attributes Learner (IAL), leveraging geo-attributes of each image for comprehensive scene perception. FlexGeo consistently outperforms existing methods on SetVL-480K and two public datasets, SeqGeo and KITTI-CVL, achieving a localization accuracy improvement of over 22% on SetVL-480K.

==> sec/4_dataset.tex <==
\section{MVL-480K Dataset}

This section introduces the key features of the proposed MVL-480K dataset, emphasizing its unique distinctions from existing datasets. We then detail its construction and evaluation protocols.

\subsection{Dataset Characteristics}

The primary aim of the MVL-480K dataset is to support the M-CVGL task, a challenge not fully addressed by previous research. Table \ref{tab
comparison} compares MVL-480K with several previous datasets for CVGL tasks, highlighting key data-level characteristics:
\begin{enumerate}
    \item \textbf{Diverse perspectives and sampling locations}: As shown in Fig. \ref{fig_sampling_comparison}, ground images in Sequence-CVGL datasets often have highly repetitive views and limited sampling locations due to the road-bound trajectories, leading to redundancy. In contrast, image sets in MVL-480K are taken from varied perspectives and locations, thus providing richer environmental information and better reflecting the conditions where users may move independently, capturing scenes from different vantage points.
    \item \textbf{Absence of Sequence Relationships Among Query Images}: Ground images in MVL-480K are captured from random perspectives, making it difficult to recover sequential information. This setup enables fair comparison among localization methods, presenting a more general and challenging geo-localization task suited to a wide range of applications.
    \item \textbf{High Query-to-Reference Image Ratio}: In MVL-480K, each reference cell is linked to an average of 40 query images. This high ratio provides ample space for researchers to extensively explore the relationship between the number of query images and localization accuracy.

\end{enumerate}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{pictures/Dataset_comparison_1024.png}
    \caption{Distribution of query data in different datasets. The left side illustrates query image distribution in S-CVGL datasets, while the right side displays the distribution in MVL-480K. The blue line indicates the vehicle's route, with blue dots as sampling points and orange markers indicating the direction of image capture.}
    \label{fig_sampling_comparison}
\end{figure*}

\subsection{Dataset Construction}

The MVL-480K dataset consists of 16,530 satellite images and 480,000 ground images, covering the central areas of six cities across different continents: Chicago, Johannesburg, London, Rio de Janeiro, Sydney, and Taipei.

The satellite images, sourced from Esri World Imagery\footnote{\url{https://www.arcgis.com/home/item.html?id=10df2279f9684e4a9f6a7f08febac2a9}}, have a \(400\times400\) resolution at zoom level 18, providing a ground resolution of approximately 0.597 meters per pixel. These images are cropped with an overlap of 0.125 for seamless coverage. Ground images, obtained using the Google Street View Static API\footnote{\url{https://developers.google.com/maps/documentation/streetview}}, have a resolution of \(512\times512\) pixels, with a limited FOV of \(90^\circ\) rather than being panoramic. Following previous datasets \cite{chen2019touchdown,muhtar2024lhrs}, we provide all the ground image IDs and the processing scripts rather than the ground images themselves\footnote{\url{https://research.google/blog/enhancing-the-research-communitys-access-to-street-view-panoramas-for-language-grounding-tasks/}}. Additionally, each reference image's latitude and longitude are collected, along with the coordinates and angles relative to true north for each query image. The training and testing sets are evenly divided, with a 1:1 ratio.

\subsection{The Evaluation Protocol}

For M-CVGL, we adopt the evaluation metrics Recall@K-N and AP-N, which are adaptations of the standard Recall@K and AP (Average Precision) metrics. The parameter N indicates the number of query images used in joint geo-localization. Recall@K measures the proportion of queries with the correct result in the top K retrieved results, reflecting model accuracy within a rank range. Recall@K-N extends this by evaluating performance when aggregating N query images, capturing both retrieval rank K and query image count N. Similarly, AP-N assesses retrieval accuracy with multiple query images.



